One-shot Empirical Privacy Estimation for Federated Learning

Privacy estimation techniques for differentially private (DP) algorithms are useful for comparing against analytical bounds, or to empirically measure privacy loss in settings where known analytical bounds are not tight. However, existing privacy auditing techniques usually make strong assumptions on the adversary (e.g., knowledge of intermediate model iterates or the training data distribution), are tailored to specific tasks, model architectures, or DP algorithm, and/or require retraining the model many times (typically on the order of thousands). These shortcomings make deploying such techniques at scale difficult in practice, especially in federated settings where model training can take days or weeks. In this work, we present a novel "one-shot" approach that can systematically address these challenges, allowing efficient auditing or estimation of the privacy loss of a model during the same, single training run used to fit model parameters, and without requiring any a priori knowledge about the model architecture, task, or DP training algorithm. We show that our method provides provably correct estimates for the privacy loss under the Gaussian mechanism, and we demonstrate its performance on well-established FL benchmark datasets under several adversarial threat models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:related}

Differential privacy provides strong guarantees for privacy of a training algorithm, but in many deployments there remains a significant gap between the formal guarantees and real-world expectations. The privacy parameters are often chosen according to worst-case analytical bounds, which need to ensure that the definition of DP is guaranteed for any dataset, any output regions of the algorithm, and adversaries of infinite abilities. Existing approaches have serious difficulties balancing provable robustness to such extreme worst-case scenarios and model utility. To obtain models that even weakly rival non-private models in accuracy, it is common to add so little noise that the empirical privacy guarantee is essentially vacuous. Many published works \citep{li2021large,anil2021large,kairouz2021practical} report $\varepsilon$ values in the range 5--20, and the U.S. Census 2020 dataset was released with $\varepsilon = 19.6$. Even the low end of this range, $\varepsilon = 5$, means that with non-negligible probability (at least $\delta$), an attacker could observe an output that lets them conclude with confidence at least $\frac{e^5}{1 + e^5} \approx 99.3\%$, the targeted user was present in the training population. On the other hand, there is a line of research providing evidence that even a small amount of noise is sufficient to significantly obscure the influence of individual users preventing reconstruction attacks~\citep{balle2022reconstructing,guo2022bounding,guo2022analyzing,bhowmick2018protection,stock2022defending}. This naturally raises the question: how much are we losing in our DP analysis by allowing such an unbounded attacker? Would our $\varepsilon$ values be significantly smaller if we could restrict the adversary to a more realistic class?

Only a handful of training algorithms have been proved to satisfy DP, e.g.,~\citep{abadi16deep,kairouz2021practical,choquette22multi}. Slight variations on those algorithms that might reasonably be expected to improve privacy properties have no known analysis. For example, it is possible in a production system to limit the participation of each user by allowing them to participate at most a certain number of times, or dividing the training into ``epochs'' during which each user can participate at most once. Such policies should, if anything, improve privacy. But so far we don't know how to take advantage of these restrictions to give lower $\varepsilon$ values. This motivates the need for methods to empirically estimate privacy that can apply in broader situations for which we have no existing analysis.

Of particular interest is the case that only the final model is released. Intuitively, seeing only the final model should significantly weaken the attacker relative to seeing all model deltas, and this is indeed known to be the case for DP-SGD when the objective is convex~\citep{feldman2018privacy}. In centralized applications of user-level DP, only the final model (or predictions of the final model) are likely to be released. In cross-device FL, an attacker with a fleet of compromised devices could potentially access some number of intermediate updates. To successfully mount such an attack, a significant fraction of devices would have to be compromised, which becomes very difficult in production-scale FL tasks with $10^5$--$10^8$ users. The danger of this attack could also be mitigated by the use of Trusted Execution Environments on clients and on the server, allowing devices to prove that they are running local training as intended and cannot access any part of program state, in particular, the parameters for the round~\citep{mo2021ppfl,mondal2021poster}. Our experimental results confirm that the privacy loss is much lower when adversaries obtain access only to the final model compared to all intermediary updates. We also demonstrate that restricted participation of clients in the federated learning training protocol has a positive impact on privacy.

In contrast to most existing work on privacy auditing~\citep{Audit-DPSGD,nasr2021adversary,BayesianEst-DP,lu2022_auditing}, our empirical auditing method reduces the number of required training runs to just one by using all canaries during regular model training, obtaining multiple, independent measurements of canary cosines with no significant performance overhead. This enables us to design an efficient privacy auditing method for federated learning. The closest related work is CANIFE~\citep{CANIFE}, whose goal is also to perform privacy auditing of federated learning models.  Compared to CANIFE, our technique requires minimal assumptions on adversarial knowledge (as the adversary crafts random canaries for poisoning model updates), and are effective for a range of adversarial models, including realistic adversaries with access only to the final model.


==> sections/relatedwork_discussion.tex <==
\section{Discussion and Related work}
\label{sec:related}

Differential privacy~\citep{DworkMNS06} provides strong guarantees for privacy of a training algorithm, but in many deployments there remains a significant gap between the formal guarantees and real-world expectations. The privacy parameters are often chosen according to worst-case analytical bounds, which need to ensure that the definition of DP is guaranteed for any dataset, any output regions of the algorithm, and adversaries of infinite abilities. Existing approaches have serious difficulties balancing provable robustness to such extreme worst-case scenarios and model utility. To obtain models that even weakly rival non-private models in accuracy, it is common to add so little noise that the empirical privacy guarantee is essentially vacuous. Many published works \citep{li2021large,anil2021large,kairouz2021practical} report $\varepsilon$ values in the range 5--20, and the U.S. Census 2020 dataset was released with $\varepsilon = 19.6$. Even at the low end of this range, $\varepsilon = 5$, means that with non-negligible probability (at least $\delta$), an attacker could observe an output that lets them conclude that with probability at least $\frac{e^5}{1 + e^5} \approx 99.3\%$, the targeted user was present in the training population. On the other hand, there is a line of research providing evidence that even a small amount of noise is sufficient to significantly obscure the influence of individual users preventing reconstruction attacks~\citep{balle2022reconstructing,guo2022bounding,guo2022analyzing,bhowmick2018protection,stock2022defending}. This naturally raises the question: how much are we losing in our DP analysis by allowing such an unbounded attacker? Would our $\varepsilon$ values be significantly smaller if we could restrict the adversary to a more realistic class?

Only a handful of training algorithms have been proved to satisfy DP. Slight variations on those algorithms that might reasonably be expected to improve privacy properties have no known analysis. For example, it is possible in a production system to limit the participation of each user by allowing them to participate at most a certain number of times, or dividing the training into ``epochs'' during which each user can participate at most once. Such policies should, if anything, improve privacy. But no analysis has been devised that can take advantage of these restrictions to give lower $\varepsilon$ values. Of particular interest is the case that only the final model is released. Intuitively, seeing only the final model should significantly weaken the attacker relative to seeing all model deltas, and this is indeed known to be the case when the objective is convex [cite]. This motivates the need for methods to empirically estimate privacy that can apply in broader situations for which we have no existing analysis.

Privacy auditing, introduced by \citet{Audit-DPSGD}, aims to close this gap by providing techniques for empirically auditing the actual privacy leakage of an algorithm and estimating the $\varepsilon$ privacy parameter. The main technique used for privacy auditing is performing a membership inference attack~\citep{shokri2017membership,yeom2018privacy,LiRA}, which measures the success of the adversary at distinguishing whether a particular example was part of training or not, and translate that into an  $\varepsilon$ estimate using the DP definition directly. Using membership inference on a randomly chosen training example provides fairly low estimates of $\varepsilon$~\citep{EvaluatingDP-JE2019}, but selecting worst-case examples induces stronger estimates~\citep{BayesianEst-DP}. 

Several papers showed that data poisoning attacks, in which adversaries create worst-case examples to maximize their distinguishing success in membership inference, result in better estimates of $\varepsilon$~\citep{Audit-DPSGD,nasr2021adversary,lu2022_auditing}. These papers differ in the specifics of the data poisoning attack designed for auditing. \citet{Audit-DPSGD} craft clipping-aware data poisoning samples in the lowest SVD direction of the training data, under the assumption that the adversary has full knowledge of the training set. \citet{nasr2021adversary} create adversarial points using techniques similar to the generation of adversarial examples in a static data poisoning scenario, but they also consider adaptive poisoning in which the adversary generates poisoning samples adaptively and gradient attacks in which the adversary can poison gradients during training. \citet{lu2022_auditing} use a targeted poisoning attack on a random test point by maximizing the loss on that point relative to a set of shadow models. 

Privacy auditing methods from the literature most often train a large number of ML models, on the order of thousands~\citep{Audit-DPSGD,nasr2021adversary} or even hundred of thousands~\citep{Debugging-DP}, to obtain independent estimates of (FPR, FNR) pairs.  Once the (FPR, FNR) are collected, various statistical methods are used to estimate the privacy parameter~$\varepsilon$. The initial privacy auditing papers~\citep{Audit-DPSGD,nasr2021adversary} used Clopper-Pearson intervals, while more recently Jeffrey intervals~\citep{BayesianEst-DP} and Katz-log intervals~\citep{lu2022_auditing} have been shown to reduce variance. Tighter estimates have been designed based on  integrating directly over the privacy region~\citep{BayesianEst-DP}. \citet{BayesianEst-DP} also introduces the heuristic to include multiple samples in each of several training runs, but does not consider that for high-dimensional models even a single training run may be sufficient. In contrast to all these techniques, our empirical auditing method reduces the number of required training runs to just one by using all canaries during regular model training, obtaining multiple, independent measurements of canary cosines with no significane performance overhead. We estimate directly the mean and standard deviation of the Gaussian cosines of canary updates, which we translate to an $\varepsilon$ estimate. 

Most existing techniques for privacy auditing~\citep{Audit-DPSGD,nasr2021adversary,lu2022_auditing,BayesianEst-DP} have been designed for centralized settings, with  the exception of CANIFE~\citep{CANIFE}, suitable for privacy auditing of federated learning deployments. CANIFE operates under a strong adversarial model, assuming knowledge of all intermediary model updates, as well as local model updates sent by a subset of clients in each round of training. CANIFE crafts data poisoning canaries adaptively, with the goal of generating model updates orthogonal to updates sent by other clients in each round. They estimate per-round $\varepsilon$ values using Clopper-Pearson confidence intervals, which they then convert to a corresponding per-round $\sigma^2$, which are then composed using RDP across rounds to obtain an estimate of $\varepsilon$ for the entire training algorithm. Compared to CANIFE, our techniques require minimal assumptions on adversarial knowledge (as the adversary crafts random canaries for poisoning model updates), and are effective for realistic adversaries with access only to the final model.

%Number of models trained and statistical methods for estimating eps.



==> sections/threatmodel.tex <==
\section{Threat model}
